User guide on Hopf bifurcation and time periodic orbits with pde2path

We explain the setup for using the pde2path libraries for Hopf bifurcation and continuation of branches of periodic orbits and give implementation details of the associated demo directories. See [Uecker, Comm. in Comp. Phys., 2019] for a description of the basic algorithms and the mathematical background of the examples. Additionally we explain the treatment of Hopf bifurcations in systems with continuous symmetries, including the continuation of traveling waves and rotating waves in O(2) equivariant systems as relative equilibria, the continuation of Hopf bifurcation points via extended systems, and some simple setups for the bifurcation from periodic orbits associated to critical Floquet multipliers going through +-1.

==> cglfig1.tex <==
\begin{figure}[H]
\bce{\small 
\begin{tabular}{lp{0.73\textwidth}}
(a) BD, norm $\|u(\cdot,\cdot;r)\|_*$&(b) Example plots\\
\ig[width=0.24\textwidth, height=49mm]{figs/1dbdl2g}&
\hs{-4mm}%\ig[height=43mm]{figs/1d-pt27}
\ig[width=0.25\textwidth,height=49mm]{figs/b1-27}
\ig[width=0.21\textwidth]{./figs/c5-1}
\ig[width=0.25\textwidth,height=49mm ]{figs/b2-19}
%\ig[width=0.23\textwidth,height=45mm]{figs/b3-17} 
\end{tabular}
\begin{tabular}{p{0.55\textwidth}p{0.4\textwidth}}
(c) Multipliers at b1/pt8 ($\ind=1$) and b2/pt5 ($\ind=3$) (left),  
and at b1/pt27 ($\ind=0$) (right)
&{\small (d) left: BD, period $T(r)$. Right: numerical periods (for $m=20,40,60$) and analytical period (black dots) on the 1st branch} \\[1mm]
\raisebox{15mm}{\begin{tabular}{l}
\ig[height=30mm]{figs/1db1-fl8}\\[-7mm]
\raisebox{10mm}{\ig[height=25mm]{figs/1db2-fl5}}
\end{tabular}}
\raisebox{10mm}{\ig[height=30mm]{figs/1db1-fl27}}
&\ig[width=35mm,height=49mm]{figs/1dbdTa}\ig[width=35mm,height=49mm]{figs/1dbdTd}
\end{tabular}
}
\ece 

\vs{-18mm}
   \caption{{\small Selected outputs from {\tt cmds1d.m}, i.e., numerical bifurcation diagrams, example plots 
and (leading 20) Floquet multipliers 
for \reff{cAC} on the domain 
$\Om=(-\pi,\pi)$ with Neumann BC, 30 grid--points in $x$.  
Parameters $(\nu,\mu,c_3,c_5)=(1,0.1,-1,1)$, 
hence bifurcations at (restricting to the first three branches) 
$r=0$ ($k=0$, spatially homogeneous branch, black), 
$r=1/4$ ($k=1/2$, blue) and $r=1$ ($k=1$, red). 
The thick part of the black line in (a) 
indicates the only stable periodic solutions. 
 The black dots in (a) and (d) are from the (spatially homogeneous) analytical solution, see \cite{hotheo}.
For $m=20$ there is a visible error in $T$. 
The right panel of (d) shows the numerical $T$ for different $m$ ($m=20$ black, 
$m=40$ red-dashed, $m=60$ blue-dotted), which 
illustrates the convergence of the numerical solution towards the analytical solution \reff{cACs}. Similarly, the periods also converge on the other 
branches (see {\tt cmds1dconv.m}). The second plot in (b) 
shows a time series at the point {\tt p.hopf.x0i} from {\tt b1/pt27}. 
See also Fig.~\ref{f1b}(b) for a plot of {\tt b3/pt17}. 
  \label{f1}}}
\end{figure}

==> dapp.tex <==
\section{Some background and formulas}
For details and background on the basic algorithms for Hopf branch point 
(HBP) detection and localization, branch--switching to and continuation 
of Hopf orbits, and Floquet multiplier computations we refer to \cite{hotheo}. 
However, in \S\ref{appa} we first briefly repeat the pertinent formulas that are implemented 
in \pdep, including the augmented systems for Hopf computations 
with constraints. We focus on the arclength parametrization 
setting ({\tt p.sw.para=4}), which is more convenient and robust than 
the 'natural parametrization' ({\tt p.sw.para=3}). 
In \S\ref{appb} we then give the formulas used for branch--switching 
as multipliers go through $\pm 1$. We mix the presentation of 
formulas with their \pdep implementation, and in \S\ref{appd} we give an 
overview of the used data structures and functions.  


\subsection{Basics}\label{appa} 
First of all, the detection of Hopf bifurcation points (HBPs) requires the 
{\tt p.sw.bifcheck=2} setting \cite[\S2.1]{hotheo}, which is essentially controlled as follows:
{\small
\huga{
\begin{split}
&\text{{\tt p.nc.eigref(1:ne)} contains shifts near which eigenvalues are computed; guesses for these shifts}\\
&\text{ can be obtained via {\tt initeig}. However, except for \S\reff{brusec},  here we use {\tt p.nc.eigref=0}.) }
\end{split}\label{eigref}\\
\label{mus}
\begin{split}
&\text{A bisection for localization of a possible HBP is started 
if $|\re \mu|<{\tt p.nc.mu1}$ for the eigenvalue with}\\
&\text{ the smallest abs.~real part, and a HBP is accepted if $|\re\mu|<{\tt p.nc.mu2}$ at the end of the bisection.}
\end{split}
}
}
The default branch switching {\tt hoswibra} to a Hopf branch generates 
\def\dlam{\del_\lam}\def\dsd{{\rm d}s}
\huga{\label{hoswitr} 
\lam=\lam_H+\del_s\dlam
\quad u(t)=u_0+2\al\del_s\Re(\er^{-\ri \om_H t}\Psi), }
as an initial guess for a periodic solution of \reff{tformd} 
with period near $2\pi/\om$. Here $\Psi$ is the (complex) eigenvector 
associated to $\ri\om_H$, and $\del_\lam,\al$ are computed from 
the normal form 
\huga{\label{honf2}
0=r\bigg[\mu_r'(\lam_H)(\lam-\lam_H)+c_1|r|^2\bigg]. 
} 
of the bifurcation equation on the center manifold, see \cite[\S2.2]{hotheo}. After the coefficients $\del_\lam$ and $\al$ in \reff{hoswitr} are computed 
(in {\tt hogetnf}), 
$\del_s$ is chosen in such a way that the initial step length is {\tt ds} in the norm \reff{xinorm} below. 

This so far applies to semilinear systems, i.e., in FEM form 
$M\dot u=Ku-Mf(u)$ where the stiffness matrix $K$ does not depend on $u$. 
For more general problems, or in general as an alternative to the computation of $\del_\lam$ and $\al$, the 
user can also pass values for $\del_\lam$ and $\al$ 
to {\tt hoswibra}. Often, $\del_\lam=0$ (and then automatically $\al=1$ 
by normalization) works fine. 


To compute Hopf orbits, after rescaling $t\mapsto Tt$ with unknown period $T$, the time evolution and periodicity condition for $u$ read 
\huga{\label{tform3} 
M\dot u=-TG(u,\lam), \quad u(\cdot,0)=u(\cdot,1), 
}
and the time-translational phase condition and arclength equation read 
\hual{\label{pca}
\phi&:=\xi_\phi\int_0^1\spr{u(t),\dot u_0(t)}\dd t\stackrel !=0, \\
\label{ala}\psi&:=
\hoxi\sum_{j=1}^m\spr{u(t_j){-}u_0(t_j),u_0'(t_j)}_\Om+
(1{-}\hoxi)\bigl[w_T(T{-}T_0)T_0'+(1{-}w_T)(\lam{-}\lam_0)\lam_0'\bigr]{-}\rds
\stackrel!=0,
}
where $T_0,\lam_0$ and $u_0$ are from the previous step, 
$\hoxi, w_T$ are weights,  $'$ denotes differentiation wrt arclength, 
and $\spr{u,v}_\Om$ stands for $\int_\Om \spr{u(x),v(x)}\dd x$, 
with $\spr{a,b}$ the standard $\R^N$ scalar product.%
\footnote{By default ({\tt p.hopf.y0dsw=2}), $\dot u_0$ in \reff{pca} is evaluated (in {\tt sety0dot})  by 2nd order finite differences; 
alternatively, {\tt p.hopf.y0dsw=1} means first order FD, and 
{\tt p.hopf.y0dsw=0} replaces $\dot u_0$ by $M\dot u_0=-TG(u_0,\lam_0)$.}
Numerically, we use $\spr{u,v}_\Om=\spr{Mu,v}$, where $M$ is the mass matrix 
belonging to the FEM mesh.  The steplength is {\tt ds} in the weighted norm 
\huga{\label{xinorm}
\|(u,T,\lam)\|_\xi=\sqrt{\hoxi\left(\sum_{j=1}^m \|u(t_j)\|_2^2\right)+(1-\hoxi)
\bigl[w_TT^2+
(1-w_T)\lam^2\bigr]}. 
}

In \reff{pca}, $\xi_\phi$ with standard setting $\xi_\phi=10$ 
({\tt p.hopf.pcfac}, see Appendix B)  is another weight, 
which can be helpful to balance the Jacobian $\CA$, see \reff{news}. 
To improve convergence of Newton loops, it sometimes turns out to be usefull to set $\xi_\phi$ to somewhat larger values. 
Also, while $\dot u_0$ in \reff{pca} is in principle 
available from $M\dot u_0=-TG(u_0,\lam_0)$ (which is used 
for {\tt p.hopf.y0dsw=0}, it often appears more robust 
to explicitly approximate $\dot u_0$ via finite differences, 
for which we set {\tt p.hopf.y0dsw=2}. Finally, 
for a system with $n_H$ Hopf constraints 
$Q_H(u)=0$, and hence $n_H$ additional free parameters $w\in\R^{n_H}$, 
we also add $w_w\spr{w-w_0,w'}$ to $\psi$, where $w_w$ is a weight for 
the auxiliary parameters $w$. 

Letting $U=(u,T,\lam,w)$, and writing $\CG(U)=0$ for \reff{tform3} (see also 
\reff{gjdef}), in each continuation step we need to solve 
\huga{\label{fsac} 
H(U):=\bpm \CG(U)\\\phi(u)\\\psi(U)\\Q_H(U)\epm\stackrel{!}{=}\bpm 0\\0\\0\\0\epm
\in\R^{mn_u+2+n_H}, }
where $m$ is the number of time slices $t_j$, $j=1,\ldots,m$, $n_u$ the number of PDE unkowns at 
each time slice, and $n_H=:{\tt p.hopf.nqh}$ is the number of Hopf constraints 
(encoded in {\tt p.hopf.qfh}). To solve \reff{fsac} we use Newton's method, i.e., 
\huga{\label{news} 
U^{j+1}{=}U^{j}{-}\CA(U^j)^{-1}H(U^j), \quad 
\CA{=}\bpm \pa_u \CG&\pa_T\CG&\pa_\lam\CG&\pa_a \CG\\
\pa_u\phi&0&0&0\\
\hoxi\tau_u&(1{-}\hoxi)w_T\tau_T&(1{-}\hoxi)(1{-}w_T)\tau_\lam&w_a\tau_a\\
\pa_uQ_H&\pa_T Q_H&\pa_\lam Q&\pa_aQ_H
\epm, 
}
where of course we never form $\CA^{-1}$ but instead use {\tt p.fuha.blss} 
to solve linear systems of type $\CA U=b$. These systems are of bordered 
type, and thus it is often advantageous to use bordered system solvers, 
see \cite{lsstut}. 

For the time discretization we have 
\hual{\label{ydef0}
&u=(u_1,\ldots,u_m)=(u(t_1), u(t_2),\ldots, u(t_m)),\\
&\text{($m$ time slices, stored in {\tt p.hopf.y(1:p.nu,1:m)),}}\notag 
} 
where $u_m=u1$ is redundant but convenient. To assemble $\CG$ in \reff{tform3} we 
use modifications of TOM, yielding, with  $h_j=t_j-t_{j-1}$ and $u_0:=u_{m-1}$, 
\huga{\label{gjdef}
(\CG(u))_j=-h_{j-1}^{-1}M(u_j-u_{j-1})-\frac 1 2 T(G(u_j)+G(u_{j-1})), 
\quad \CG_m(u)=u_m-u_1.
}
The Jacobian is $\pa_u\CG=A_1$, where  we set, 
as it is also used for the Floquet multipliers with free $\ga$ (see \cite[\S2.4]{hotheo} and \S\ref{appb}), 
%\def\id{\bullet} 
\renewcommand{\arraystretch}{1.5}
\huga{\label{fl0}
A_\ga=
\bpm M_1&0&0&0&\ldots&-H_1&0\\
-H_2&M_2&0&0&\ldots&0&0\\
0&-H_3&M_3&0&\ldots&0&0\\
\vdots&\ldots&\ddots&\ddots&\ddots&\vdots&\vdots\\
0&\ldots&\ldots&\ddots&\ddots&0&0\\
0&\ldots&\ldots&0&-H_{m-1}&M_{m-1}&0\\
-\ga\,I&0&\ldots&\ldots&\ldots&0&I
\epm,}
\renewcommand{\arraystretch}{1}
where $\ds M_j=-h_{j-1}^{-1}M-\frac 1 2 T \pa_uG(u_j)$, 
$\ds H_j=-h_{j-1}^{-1}M+\frac 1 2 T \pa_uG(u_{j-1})$, and $I$ is 
the ${n_u\times n_u}$ identity matrix.%
\footnote{In \reff{gjdef} and \reff{fl0} we assume that $M$ is regular, 
i.e., \reff{tform3} does not contain algebraic constraints as for instance 
for the 2nd order system formulation of the KS in {\tt kspbc2}; see also Remark  \ref{flremc} for this case.} 
The Jacobians $\pa_uG\in\R^{n_u\times n_u}$ in $M_j, H_j$ are computed 
as for steady state problems, e.g., via {\tt p.fuha.sGjac}, or 
by {\tt numjac} if {\tt p.sw.jac}=0 (but still locally in time). 

For $Q_H(u(\cdot,\cdot),\lam,w,a)=0$, the user 
must provide a function handle {\tt p.hopf.qfh}, similar to 
$0=Q(u,\lam,w)={\tt p.fuha.qf}$ for the steady case. 
Moreover, when switching to a Hopf branch (and if {\tt p.nc.nq} was greater 
$0$ for 
the steady continuation), the user has to drop 
the stationary constraints, i.e., reset {\tt p.nc.nq=0} and 
{\tt p.nc.ilam=p.nc.ilam(1)} to just 
the primary active parameter, while the other active 
parameters $a\in \R^{n_H}$ for $Q_H$ should be set in 
${\tt p.hopf.ilam}\in \N^{n_H}$, which now acts as a pointer to these 
'secondary' active parameters. 
Finally, the user must provide a function handle in {\tt p.hopf.qfhjac} 
to a function that returns $\pa_u Q_H$ from the last line in \reff{news}. 
On the other hand, $\pa_T \CG, \pa_\lam \CG, \pa_a\CG$, and $\pa_TQ_H, \pa_\lam Q_H$ 
and $\pa_a Q_H$ in \reff{news} are cheap from 
numerical differentiation and hence taken care of automatically. 



\brem\label{flremc}{\rm 
 If \reff{tform3} contains algebraic constraint components as 
in {\tt kspbc2}, then we modify \reff{gjdef}. For instance, 
if the second component is algebraic, then we (automatically, 
in {\tt tomassemF} and {\tt tomassempbc}) set 
$(\CG(u)_2)_j=-\frac 1 2 TG(u_j)$, and accordingly also modify 
\reff{fl0}. 
%Also in this case we still use $A_\ga$ to compute Floquet multipliers, allthough this 
} \eex\erem 

\subsection{Floquet multipliers, and bifurcation from periodic orbits}\label{appb} 
\def\gacrit{\ga_{{\rm crit}}}
The Floquet multipliers $\ga$ of a periodic orbit $u_H$ are obtained 
 from 
finding nontrivial solutions $(v,\ga)$ of the variational boundary value 
problem 
\hual{
M\dot v(t)&=-T\pa_u G(u(t))v(t),\label{fl1}\\ 
v(1)&=\ga v(0).
}
By translational invariance of \reff{tform3}, there always is the trivial multiplier $\ga_1=1$. 
Equivalently, the multipliers $\ga$ are the eigenvalues of 
the monodromy matrix $\CM(u_0)=\pa_u \Phi(u_0,T)$, where $\Phi(u_0,t)$ is 
the solution of the initial value problem \reff{tform3} with $u(0)=u_0$ 
from $u_H$. 
Thus, $\CM(u_0)$ depends on $u_0$, but the multipliers $\ga$ do not. 
$\CM(u_0)$ has the eigenvalues $1,\ga_2,\ldots,\ga_{n_u}$, where 
$\ga_2,\ldots,\ga_{n_u}$ are the multipliers of the linearized Poincar\'e map 
$\Pi(\cdot; u_0)$, which maps a point $\ut_0$ in a hyperplane 
$\Sigma$ through $u_0$ and transversal to $u_H$ to its first return to $\Sigma$, see, e.g., \cite[Theorem 1.6]{kuz04}. 
Thus, a necessary condition for the bifurcation 
from a branch $\lam\mapsto u_H(\cdot,\lam)$ of periodic orbits 
is that at some $(u_H(\cdot,\lam_0),\lam_0)$, 
additional to the trivial multiplier $\ga_1=1$ there is a 
second multiplier $\gacrit=\ga_2$ (or a complex conjugate pair $\ga_{2,3}$) 
with $|\ga_2|=1$, which generically leads to the following bifurcations 
(see, e.g., \cite[Chapter 7]{seydel} or \cite{kuz04} for more details): 
\bci
\item[(i)]\label{biftypes} $\ga_2=1$, yields a fold of the periodic orbit, or a transcritical or pitchfork bifurcation of periodic orbits.
\item[(ii)] $\ga_2=-1$, yields a period--doubling bifurcation, i.e., the bifurcation 
of periodic orbits $\ut(\cdot;\lam)$ with approximately double the period, 
$\ut(\tilde T;\lam)=\ut(0;\lam)$, $\tilde{T}(\lam)\approx 2T(\lam)$ for 
$\lam$ near $\lam_0$.  
\item[(iii)] $\ga_{2,3}=\er^{\pm\ri \vt}$ , $\vt\ne 0,\pi$, 
yields a torus (or Naimark--Sacker) bifurcation, i.e., the bifurcation 
of periodic orbits $\ut(\cdot,\lam)$ with two ``periods'' $T(\lam)$ and 
$\tilde T(\lam)$; 
if $T(\lam)/\tilde T(\lam)\not\in \Q$, then $\R\ni t\mapsto \ut(t)$ is dense in 
certain tori.  
\eci 
Numerics for (iii) are difficult even for low dimensional ODEs, but 
there are various algorithms for (i),(ii), and below we explain the simple ones 
so far used in \pdep. 
First we are interested in the computation of the multipliers. 
Using the same discretization for $v$ as for $u$, it follows that $\ga$ 
and $v=(v_1,\ldots,v_m)$ have to satisfy 
\huga{\label{fl2}
v_1=M_1^{-1}H_1v_{m-1},\quad v_2=M_2^{-1}H_2v_1,\quad \ldots,\quad v_{m-1}=M_{m-1}^{-1}H_{m-1}v_{m-2},\quad v_m=\ga v_1, 
}
for some $\ga\in\C$. 
Thus, $\CM(u_{j_0})$ can be obtained 
from certain products involving the $M_j$ and the $H_j$, for instance%
\footnote{In \cite[(2.40)]{hotheo} we used $\CM(u_{m-1})$, but $\CM(u_{1})$ 
seems more convenient for branch--switching}
\huga{\label{fl3} 
\CM(u_{1})=M_1^{-1}H_1M_{m-1}^{-1}H_{m-1}\cdots M_2^{-1}H_2. 
} 
Thus, a simple way to compute the $\ga_j$ is to compute the 
product \reff{fl3} and subsequently  (a number of) 
the eigenvalues of $\CM(u_{1})$. We call this \fla\ (Floquet Algorithm 1, 
implemented in {\tt floq}), and using 
\huga{\label{emudef}
\emu:=|\ga_1-1|} 
as a measure of accuracy we find that this works 
fast and accurately for our dissipative examples. Typically 
$\emu<10^{-10}$, although at larger amplitudes of $u_H$, 
and if there are large multipliers, this may 
go up to $\emu\sim 10^{-8}$, which is the (default) tolerance we require 
for the computation of $u_H$ itself. Thus, in the software 
 we give a warning if $\emu$ exceeds a certain tolerance 
$\fltol$.   
However, for the optimal control example in \S\ref{ocsec}, 
where we naturally have multipliers $\ga_j$ with 
$|\ga_j|>10^{30}$ and larger, 
\fla\ completely fails to compute any meaningful multipliers. 


More generally, in for instance \cite{fj91,lust01} it is explained that methods 
based directly on \reff{fl3} 
\bci
\item%
may give considerable numerical errors, in particular if 
there are both, very small and very large multipliers $\ga_j$; 
\item%
discard much useful information, for instance eigenvectors 
of $\CM(u_l)$, $l\ne m-1$, which are useful for branch switching.
\eci
As an alternative, \cite{lust01} suggests to use a periodic Schur decomposition 
\cite{BGD93} to compute the multipliers (and subsequently 
pertinent eigenvectors), and gives examples that in certain cases 
this gives much better accuracy, according to \reff{emudef}. 
See also \cite{kressner01, kress06} for similar ideas and results. 
We thus provide an algorithm \flb\  (Floquet Algorithm 2, 
implemented in {\tt floqps}), 
which, based on {\tt pqzschur} from \cite{kressner01}, 
computes a periodic Schur decomposition of the matrices involved 
in \reff{fl3}, from which we immediately obtain the multipliers, see 
\cite{hotheo} for details. 

\brem\label{flremd}{\rm 
Also for $n_H>0$, the computation of Floquet multipliers is based on \reff{fl0}, 
i.e., ignores the Hopf-constraints $Q_H$. Since these constraints are 
typically used to eliminate neutral directions, ignoring these typically 
leads to Floquet multipliers close to $1$, additional to the trivial 
multiplier $1$ from (time--) translational invariance. This may lead to 
wrong stability assessments of periodic orbits (see \cite[\S4]{symtut} 
for an example), which however usually can identified by suitable 
inspection of the multipliers. 
} \eex\erem 

Here, additional to \cite{hotheo}, we give the (somewhat preliminary, 
see Remark \ref{bsprem}) algorithms for branch 
switching for the case of $\gacrit=\pm 1$. 
First, the (simple) localization 
of a BP is done in {\tt hobifdetec.m} via bisection. 
For the case $\gacrit=1$ with associated eigenvector 
$v_1$ (i.e., $\gacrit\approx 1$ but not equal to the trivial 
multiplier, and hence $v_1\ne \pa_t u_H(0)$) 
we then use \reff{fl3}, i.e., 
\huga{\label{fl2b}
v_2=M_2^{-1}H_2v_1,\quad \ldots,\quad v_{m-1}=M_{m-1}^{-1}H_{m-1}v_{m-2},
}
and additionally $v_m=v_1$, to obtain a tangent predictor 
$V=(v_1,v_2,\ldots,v_{m-1}|v_m)$ for the bifurcating branch. 

For the case $\gacrit=-1$ we double the period $T$, i.e., set 
(recall that $t_1=0$) 
\huga{t_{{\rm new}}=\frac 1 2 (t_1,t_2,t_3,\ldots,t_{m-1},1+t_1,1+t_2,\ldots,
1+t_{m-1}), 
} 
redefine $m=2m$, and use 
$(V,-V|v_1)$ with $V$ from \ref{fl2b} as predictor. The pertinent 
function is {\tt poswibra.m}, which, besides the orbit and branch point, 
and the new directory and the (initial) step length {\tt ds}, can 
take some additional arguments {\tt aux}. For instance, {\tt aux.sw=1} 
{\em forces} {\tt poswibra} to take $\gacrit$ from near $1$, while 
{\tt aux.sw=-1} takes $\gacrit$ from near $-1$. This is sometimes 
necessary because there may be $\ga_j$ close to both, $\pm 1$, 
and the bisection for the localization does not distinguish these 
(or even multipliers elsewhere near the unit circle). 


\section{Data structure and function overview}
\label{appd}
The  Hopf setting naturally reuses and extends the stationary \pdep\ setting 
explained in, e.g., \cite{qsrc}. As usual, here we assume that the problem 
is described by the struct {\tt p}, and for convenience list the main 
subfields of {\tt p}  in Table \ref{tab1a}. 

{\small
\begin{longtable}{|p{0.07\textwidth}|p{0.38\textwidth}|
p{0.07\textwidth}|p{0.38\textwidth}|}
\caption{{Main fields in the structure {\tt p} for steady problems, see \cite{qsrc} 
for more details.
}\label{tab1a}}
\endfirsthead\endhead\endfoot\endlastfoot
\hline
field&purpose&field &purpose\\\hline
fuha&{\bf fu}nction {\bf ha}ndles, e.g., fuha.G, \ldots& nc&
{\bf n}umerical {\bf c}ontrols, e.g., nc.tol, \ldots\\
sw&{\bf sw}itches such as sw.bifcheck,\ldots&
sol&values/fields calculated at runtime\\
pdeo&OOPDE data if OOPDE is used&
mesh&mesh data (if the {\tt pdetoolbox} is used)\\
plot&switches and controls for plotting&file&switches etc for file output\\
bel&controls for lssbel (bordered elimination)&ilup&controls for lssAMG 
(ilupack parameters)\\ 
\hline
usrlam&\multicolumn{3}{p{0.85\textwidth}|}{vector of user set target 
values for the primary parameter, default usrlam=[];} \\
mat&\multicolumn{3}{p{0.75\textwidth}|}
{problem matrices, in general data that is not saved to file}\\
\hline
\end{longtable}
}

For the continuation of time-periodic orbits, the field {\tt p.hopf} contains the pertinent data; it is typically created and filled by calling {\tt p=hoswibra(..)}. This inter alia  calls {\tt p=hostanparam(p,aux)}, which 
can be used as a reference for the default values of the Hopf parameters. 
The unconstrained Hopf setting does not need any user setup additional to the 
functions such as {\tt p.fuha.sG, p.fuha.sGjac} already needed for stationary problems. In case of Hopf constraints, 
the user has to provide two function handles in {\tt p.hopf.qfh} and 
{\tt p.hopf.qfhder} to functions which compute $Q_H$ from \reff{fsac} 
and the last row of $\CA$ from \reff{news}, respectively. 
The only changes of the core {\tt p2p} library concern some queries 
whether we consider a Hopf problem, in which case basic 
routines such as {\tt cont} call a Hopf version, i.e., {\tt hocont}. 
Table \ref{hotab1} gives an overview of {\tt p.hopf}, and 
Table \ref{hotab2} lists the main Hopf orbit related functions. 

%\clearpage

% HBPs are flagged by {\tt p.sol.ptype=3}, while points on a 
% Hopf branch have {\tt p.sol.ptype=4}. The natural parametrization 
% (\S\ref{natpasec}) for periodic orbit continuation 
% is flagged by {\tt p.sw.para=3}, while 
% {\tt p.sw.para=4} flags arclength (\S\ref{alsec}). 


%\LTcapwidth=\textwidth\setlength{\LTpre}{2mm}\setlength{\LTpost}{0pt}
{\small 
\begin{longtable}{|p{0.16\tew}|p{0.84\tew}|}
\caption{Standard (and additional, at bottom) entries in {\tt p.hopf}.\label{hotab1}}
\endfirsthead\endhead\endfoot\endlastfoot
\hline
field&purpose\\
\hline
y&for {\tt p.sw.para=4}: unknowns in the form ($u=(u_1,\ldots,u_m)=(u(t_1), u(t_2),\ldots, u(t_m))$,
\text{ ($m$ time slices, y=$n_u\times m$ matrix);} \\
&for {\tt p.sw.para=3}: $y$ augmented by $\tilde y$ and $T,\lam$ 
($(2n_u{+}2)\times m$ matrix), see \cite{hotheo}.  \\
y0d&for {\tt p.sw.para=4}: $M\dot u_0$ for the phase condition \reff{pca}, 
 ($n_u\times m$ matrix); \\
&for {\tt p.sw.para=3}: $M\dot u_0(0)$  for the phase condition 
\cite[(36)]{hotheo},
($2n_u{+}2$ vector). \\
y0dsw&(for {\tt p.sw.para=4}) controls how $\dot u_0$ in \reff{pca} is computed: 0 for using the PDE \reff{tform3}, 2 for using FD (default).\\
pcfac&weight for the phase condition \reff{pca}, default=10\\
tau&tangent, for {\tt p.sw.para=4}, $(mn_u+2+n_H)\times 1$ vector, see third line in \reff{news}\\
ysec&for {\tt p.sw.para=3}, secant between two solutions $(y_0,T_0,\lam_0)$, $(y_1,T_1,\lam_1)$, $(2n_u{+}2)\times m$ matrix\\
sec&if sec=1, then use secant tau (instead of tangent) predictor for {\tt  p.sw.para=4}\\
t, T, lam&time discretization vector, current period and param.value\\
xi,tw,qw&weights for the arclength \reff{ala}, xi=$\hoxi$, tw=$w_T$, qw=$w_a$; \\
x0i&index for plotting $t\mapsto u(\vx({\tt x0i})$;\\
plot&aux. vars to control hoplot during hocont; see the description of {\tt hoplot}; default plot=[]\\
wn&struct containing the winding number related settings for {\tt initeig}\\
tom&struct containing TOM settings, including the mass matrix $M$\\
jac&switch to control assembly of $\pa_u\CG$. jac=0: numerically (only recommended for testing); jac=1: via {\tt hosjac}.  Note 
that for {\tt p.sw.jac=0} the local matrices $\pa_u G(u(t_j))$ are 
obtained via {\tt numjac}, but this is still much faster than using {\tt p.hopf.jac=0}. \\
flcheck&0 to switch off multiplier-comp.~during cont., 1 to use 
{\tt floq}, 2 to use {\tt floqps}\\
nfloq&\# of multipliers (of largest modulus) to compute (if flcheck=1)\\
fltol& tolerance for multiplier $\ga_1$ 
(give warning if $|\ga_1-1|>${\tt p.hopf.fltol})\\
muv1,muv2&vectors of stable and unstable multipliers, respectively\\
pcheck&if 1, then compute residual in hoswibra (predictor check)\\
bisec&\# of bisection used for BP localizations\\
%scf&scaling factor for \reff{tform3}\\
\hline
&\hs{30mm}Additional entries in case of Hopf constraints\\
\hline 
ilam&pointer to the $n_Q$ additional active parameters in {\tt p.u(p.nu+1:end)}; the pointer to the primary active parameter is still in {\tt p.nc.ilam(1)}. \\
qfh, qfhder&(handles to) functions returning the Hopf constraints $Q_H(U)$ and 
the derivatives (last lines of $H$ in \reff{fsac} and $\CA$ in \reff{news}, 
respectively). \\
\hline
spar,kwnr&index of speed paramater, and spatial wave-nr for TW continuation, 
set in twswibra\\
\hline
\end{longtable}
}
%The unconstrained Hopf setting does not need any user setup additional to the functions such as {\tt p.fuha.sG, p.fuha.sGjac} already needed to describe stationary problems. 

{\small 
\begin{longtable}{|p{0.2\tew}|p{0.8\tew}|} 
\caption{Overview of main functions related to Hopf bifurcations and 
periodic orbits; see {\tt p2phelp} for argument lists and more comments.
\label{hotab2}}
\endfirsthead\endhead\endfoot\endlastfoot
\hline
name&purpose, remarks\\
\hline
hoswibra&branch switching at Hopf bifurcation point, see comments below \\
twswibra&branch switching at Hopf bifurcation point to Traveling Wave branch 
(which is continued as a rel.equilibrium)\\ 
hoswipar&change the active continuation parameter, see also swiparf\\
hoplot&plot the data contained in hopf.y. Space-time plot in 1D; in 2D and 3D: 
snapshots at (roughly) $t=0$, $t=T/4$, $t=T/2$ and $t=3T/4$; see also hoplotf; \\
%p=initeig(p,ommax)&find guess for $\om_1$; auxiliary argument {\tt ommax}$=\om_\max$ in {\tt p=initeig(p,ommax)} determines the interval $[0,\om_\max)$ for 
%estimating $\om_1$; if omitted, then $\om_\max=\|G_u\|$ is used. \\
initeig&find guess for $\om_1$; see also initwn\\
floq&compute {\tt p.hopf.nfloq} multipliers during continuation 
({\tt p.hopf.flcheck}=1)\\
floqps&use periodic Schur to compute (all) multipliers during continuation 
(flcheck=2)\\
floqap, floqpsap&a posteriori versions of floq and floqps, respectively\\
hobra&standard--setting for p.fuha.outfu (data on branch), 
template for adaption to a given problem \\
hostanufu&standard function called after each continuation step\\
plotfloq&plot previously computed multipliers\\
\hline
hpcontini&init Hopf point continuation\\
hpcontexit&exit Hopf point continuation\\
hpjaccheck&check user implementation of \reff{HPC4} against finite differences\\
hploc&use extended system \reff{HPC1} for Hopf point localization\\
hobifdetec&detect bifurcations {\em from} Hopf orbits, and use bisection for localization, based on multipliers \\
poswibra&branch switching {\em from} Hopf orbits\\
hobifpred&compute predictor for branch switching {\em from} Hopf orbits\\
hotintxs&time integrate \reff{tformd} from the data 
contained in p.hopf and u0, with output of $\|u(t)-u_0\|_\infty$, 
and saving $u(t)$ to disk at specified values\\
tintplot*d&plot output of hotintxs; $x{-}t$--plots for *=1, else snapshots 
at specified times \\
hopftref&refine the $t$-mesh in the arclength setting at user 
specified time $t^*$\\
hogradinf&convenience function returning the time $t^*$ where $\|\pa_t u(\cdot,t)\|_{\infty}$ is maximal; may be useful for hopftref. \\
\hline
initwn&init vectors for computation of initial guess for spectral shifts $\om_j$\\
hogetnf&compute initial guesses for dlam, al from the normal form  coefficients of bifurcating Hopf branches, see \cite[(16)]{hotheo}\\
hocont&main continuation routine; called by cont if p.sol.ptype$>$2\\
%hospcalc&called by hoswibra to compute eigenvalues near the imag.axis\\
hostanparam&set standard parameters \\
hostanopt&set standard options for hopf computations\\
hoinistep&perform 2 initial steps and compute secant, used if {\tt p.sw.para=3}\\
honloopext,honloop&the arclength Newton loop, and the Newton loop with fixed $\lam$\\
sety0dot&compute $\dot u_0$ for the phase condition \reff{pca}\\
tomsol&use TOM to compute periodic orbit in p.sw.para=3 setting.\\
tomassemG&use TOM to assemble $\CG$, see \cite[(26)]{hotheo}; see also 
{\tt tomassem, tomassempbc} \\
%or $(\CG,\pa_u\CG, \pa_T\CG,\pa_\lam\CG)$, respectively\\
%tomassempbc&pad $y$ and assemble with periodic BC; calls tomassemG and tomassem\\
gethoA&put together the extended Jacobian $\CA$ from \cite[(27)]{hotheo}\\
hopc&the phase condition $\phi$ from\cite[(19)]{hotheo},  
and $\pa_u\phi$.  \\
arc2tom, tom2arc&convert arclength data to tomsol data, e.g., to call tomsol for mesh adaptation. tom2arc to go back. \\
ulamcheckho&check for and compute solutions at user specified values in 
p.usrlam\\
\hline
hosrhs,hosrhsjac&interfaces to p.fuha.G and p.fuha.Gjac at fixed $t$, internal functions called by tomassempbc, together with hodummybc\\
horhs,hojac&similar to hosrhs, horhsjac, for p.sw.para=3, see also {\tt hobc} 
and {\tt hobcjac}\\
\hline
\end{longtable}
}

Besides {\tt cont}, the functions 
{\tt initeig}, {\tt hoswibra}, {\tt poswiba}, {\tt hoplot}, {\tt twswibra}, {\tt floqap}, 
{\tt floqplot}, {\tt hotintxs}, {\tt tintplot*d},  and {\tt hopftref}  are 
most likely to be called directly by the user, 
and {\tt hobra} (the branch data) and 
{\tt hostanufu} (called after each continuation step) are likely to be adapted by the user. 
As usual, all functions in Table \ref{hotab2} can be most easily overloaded 
by copying them to the given problem directory and modifying them there.  

In {\tt p=hoswibra(dir,fname,ds,para,varargin)}, 
the auxiliary argument {\tt aux=varargin$\{2\}$} \linebreak ({\tt varargin$\{1\}$} is 
the new directory)  
can for instance have the following 
fields:  
\bci
\item {\tt aux.tl}=30: 
number of (equally spaced) initial mesh-points in $t\in[0,1]$ 
(might be adaptively refined by TOM for {\tt p.sw.para=3}, or via {\tt hopftref} or 
{\tt uhopftref}  for {\tt p.sw.para=4}). 
\item {\tt aux.hodel}=1e-4: used for the finite differences in {\tt hogetnf}. 
\item {\tt aux.al, aux.dlam} (no preset): these can be used to pass a guess 
for $\al$ and $\del_\lam$ in \reff{hoswitr} and thus circumvent {\tt hogetnf}; 
useful for quasilinear problems and for problems with constraints (for 
which {\tt hogetnf} will not work), or more generally when the computation of $\al, \del_\lam$ via {\tt hogetnf} seems to give unreliable results. 
\item {\tt aux.z}: The coefficients $z_{1},\ldots,z_m$ in the ad hoc modification 
\reff{eqswibra} of \reff{hoswitr} used for Hopf points of higher multiplicity 
$m$. 
\eci 

For the other functions listed above we refer to the m-files for 
description of their arguments, and to the demo directories for 
examples of usage and customization. 


%\clearpage



